Deep Learning Applied to Chest X-Rays: Exploiting and Preventing Shortcuts

While deep learning has shown promise in improving the automated diagnosis of disease based on chest X-rays, deep networks may exhibit undesirable behavior related to shortcuts. This paper studies the case of spurious class skew in which patients with a particular attribute are spuriously more likely to have the outcome of interest. For instance, clinical protocols might lead to a dataset in which patients with pacemakers are disproportionately likely to have congestive heart failure. This skew can lead to models that take shortcuts by heavily relying on the biased attribute. We explore this problem across a number of attributes in the context of diagnosing the cause of acute hypoxemic respiratory failure. Applied to chest X-rays, we show that i) deep nets can accurately identify many patient attributes including sex (AUROC = 0.96) and age (AUROC >= 0.90), ii) they tend to exploit correlations between such attributes and the outcome label when learning to predict a diagnosis, leading to poor performance when such correlations do not hold in the test population (e.g., everyone in the test set is male), and iii) a simple transfer learning approach is surprisingly effective at preventing the shortcut and promoting good generalization performance. On the task of diagnosing congestive heart failure based on a set of chest X-rays skewed towards older patients (age >= 63), the proposed approach improves generalization over standard training from 0.66 (95% CI: 0.54-0.77) to 0.84 (95% CI: 0.73-0.92) AUROC. While simple, the proposed approach has the potential to improve the performance of models across populations by encouraging reliance on clinically relevant manifestations of disease, i.e., those that a clinician would use to make a diagnosis.

==> mlhc-submission-files/dataset_colordef.tex <==
\definecolor{DS0b0}{rgb}{0.282884,0.135920,0.453427}
\definecolor{DS0f0}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b1}{rgb}{0.265145,0.232956,0.516599}
\definecolor{DS0f1}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b2}{rgb}{0.150476,0.504369,0.557430}
\definecolor{DS0f2}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b3}{rgb}{0.945636,0.899815,0.112838}
\definecolor{DS0f3}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS0b4}{rgb}{0.246070,0.738910,0.452024}
\definecolor{DS0f4}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b5}{rgb}{0.327796,0.773980,0.406640}
\definecolor{DS0f5}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS0b6}{rgb}{0.252899,0.742211,0.448284}
\definecolor{DS0f6}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b7}{rgb}{1,1,1}
\definecolor{DS0f7}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b8}{rgb}{0.277941,0.056324,0.381191}
\definecolor{DS0f8}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b9}{rgb}{0.180629,0.429975,0.557282}
\definecolor{DS0f9}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b10}{rgb}{0.151918,0.500685,0.557587}
\definecolor{DS0f10}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS0b11}{rgb}{0.227802,0.326594,0.546532}
\definecolor{DS0f11}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b0}{rgb}{0.275191,0.194905,0.496005}
\definecolor{DS1f0}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b1}{rgb}{0.220057,0.343307,0.549413}
\definecolor{DS1f1}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b2}{rgb}{0.140536,0.530132,0.555659}
\definecolor{DS1f2}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b3}{rgb}{0.935904,0.898570,0.108131}
\definecolor{DS1f3}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS1b4}{rgb}{0.344074,0.780029,0.397381}
\definecolor{DS1f4}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS1b5}{rgb}{0.555484,0.840254,0.269281}
\definecolor{DS1f5}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS1b6}{rgb}{0.311925,0.767822,0.415586}
\definecolor{DS1f6}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b7}{rgb}{1,1,1}
\definecolor{DS1f7}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b8}{rgb}{0.280894,0.078907,0.402329}
\definecolor{DS1f8}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b9}{rgb}{0.150476,0.504369,0.557430}
\definecolor{DS1f9}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b10}{rgb}{0.194100,0.399323,0.555565}
\definecolor{DS1f10}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS1b11}{rgb}{0.258965,0.251537,0.524736}
\definecolor{DS1f11}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b0}{rgb}{0.258965,0.251537,0.524736}
\definecolor{DS2f0}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b1}{rgb}{0.190631,0.407061,0.556089}
\definecolor{DS2f1}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b2}{rgb}{0.147607,0.511733,0.557049}
\definecolor{DS2f2}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b3}{rgb}{0.993248,0.906157,0.143936}
\definecolor{DS2f3}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS2b4}{rgb}{0.281477,0.755203,0.432552}
\definecolor{DS2f4}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b5}{rgb}{0.140210,0.665859,0.513427}
\definecolor{DS2f5}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b6}{rgb}{0.128087,0.647749,0.523491}
\definecolor{DS2f6}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b7}{rgb}{1,1,1}
\definecolor{DS2f7}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b8}{rgb}{0.282656,0.100196,0.422160}
\definecolor{DS2f8}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b9}{rgb}{0.258965,0.251537,0.524736}
\definecolor{DS2f9}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b10}{rgb}{0.150476,0.504369,0.557430}
\definecolor{DS2f10}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS2b11}{rgb}{0.233603,0.313828,0.543914}
\definecolor{DS2f11}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b0}{rgb}{0.267004,0.004874,0.329415}
\definecolor{DS3f0}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b1}{rgb}{0.271305,0.019942,0.347269}
\definecolor{DS3f1}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b2}{rgb}{0.160665,0.478540,0.558115}
\definecolor{DS3f2}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b3}{rgb}{0.916242,0.896091,0.100717}
\definecolor{DS3f3}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS3b4}{rgb}{0.150148,0.676631,0.506589}
\definecolor{DS3f4}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b5}{rgb}{0.319809,0.770914,0.411152}
\definecolor{DS3f5}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS3b6}{rgb}{0.296479,0.761561,0.424223}
\definecolor{DS3f6}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b7}{rgb}{1,1,1}
\definecolor{DS3f7}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b8}{rgb}{0.267004,0.004874,0.329415}
\definecolor{DS3f8}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b9}{rgb}{0.171176,0.452530,0.557965}
\definecolor{DS3f9}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b10}{rgb}{0.121148,0.592739,0.544641}
\definecolor{DS3f10}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS3b11}{rgb}{0.194100,0.399323,0.555565}
\definecolor{DS3f11}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b0}{rgb}{0.280267,0.073417,0.397163}
\definecolor{DS4f0}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b1}{rgb}{0.283197,0.115680,0.436115}
\definecolor{DS4f1}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b2}{rgb}{0.156270,0.489624,0.557936}
\definecolor{DS4f2}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b3}{rgb}{0.935904,0.898570,0.108131}
\definecolor{DS4f3}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS4b4}{rgb}{0.252899,0.742211,0.448284}
\definecolor{DS4f4}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b5}{rgb}{0.404001,0.800275,0.362552}
\definecolor{DS4f5}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS4b6}{rgb}{0.360741,0.785964,0.387814}
\definecolor{DS4f6}{rgb}{0.000000,0.000000,0.000000}
\definecolor{DS4b7}{rgb}{1,1,1}
\definecolor{DS4f7}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b8}{rgb}{0.274952,0.037752,0.364543}
\definecolor{DS4f8}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b9}{rgb}{0.156270,0.489624,0.557936}
\definecolor{DS4f9}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b10}{rgb}{0.150476,0.504369,0.557430}
\definecolor{DS4f10}{rgb}{0.900000,0.900000,0.900000}
\definecolor{DS4b11}{rgb}{0.225863,0.330805,0.547314}
\definecolor{DS4f11}{rgb}{0.900000,0.900000,0.900000}


==> mlhc-submission-files/dataset_exp.tex <==
\resizebox{\columnwidth}{!}{\begin{tabular}{cccccccccccccccccccc} \toprule & \multicolumn{7}{c}{Independent Joint Statistics} & & \multicolumn{4}{c}{Joint Joint Statistics}\\ &   &   &   &   &   & Neck +  & Head +  &   & Fully  & Upper  & Only  & All But \\ 
 & Ankle  & Knee  & Hip  & Wrist  & Elbow  & Should.  & Face  &   & Visible  & Torso  & Arms  & Head \\ 
\midrule 
Average  &  \cellcolor{DS0b0} \textcolor{DS0f0}{ 7.0} &  \cellcolor{DS0b1} \textcolor{DS0f1}{ 12.9} &  \cellcolor{DS0b2} \textcolor{DS0f2}{ 31.9} &  \cellcolor{DS0b3} \textcolor{DS0f3}{ 71.9} &  \cellcolor{DS0b4} \textcolor{DS0f4}{ 50.8} &  \cellcolor{DS0b5} \textcolor{DS0f5}{ 53.9} &  \cellcolor{DS0b6} \textcolor{DS0f6}{ 51.1} &  \cellcolor{DS0b7} \textcolor{DS0f7}{ ~~ } &  \cellcolor{DS0b8} \textcolor{DS0f8}{ 2.8} &  \cellcolor{DS0b9} \textcolor{DS0f9}{ 26.2} &  \cellcolor{DS0b10} \textcolor{DS0f10}{ 31.8} &  \cellcolor{DS0b11} \textcolor{DS0f11}{ 18.8}\\ 
\midrule
VLOG \cite{Fouhey18}  &  \cellcolor{DS1b0} \textcolor{DS1f0}{ 10.5} &  \cellcolor{DS1b1} \textcolor{DS1f1}{ 20.0} &  \cellcolor{DS1b2} \textcolor{DS1f2}{ 34.0} &  \cellcolor{DS1b3} \textcolor{DS1f3}{ 71.5} &  \cellcolor{DS1b4} \textcolor{DS1f4}{ 54.5} &  \cellcolor{DS1b5} \textcolor{DS1f5}{ 61.0} &  \cellcolor{DS1b6} \textcolor{DS1f6}{ 53.3} &  \cellcolor{DS1b7} \textcolor{DS1f7}{ ~~ } &  \cellcolor{DS1b8} \textcolor{DS1f8}{ 4.0} &  \cellcolor{DS1b9} \textcolor{DS1f9}{ 32.0} &  \cellcolor{DS1b10} \textcolor{DS1f10}{ 24.0} &  \cellcolor{DS1b11} \textcolor{DS1f11}{ 14.0}\\ 
Instructions \cite{Alayrac2016}  &  \cellcolor{DS2b0} \textcolor{DS2f0}{ 14.0} &  \cellcolor{DS2b1} \textcolor{DS2f1}{ 24.5} &  \cellcolor{DS2b2} \textcolor{DS2f2}{ 32.5} &  \cellcolor{DS2b3} \textcolor{DS2f3}{ 73.5} &  \cellcolor{DS2b4} \textcolor{DS2f4}{ 52.0} &  \cellcolor{DS2b5} \textcolor{DS2f5}{ 44.7} &  \cellcolor{DS2b6} \textcolor{DS2f6}{ 43.3} &  \cellcolor{DS2b7} \textcolor{DS2f7}{ ~~ } &  \cellcolor{DS2b8} \textcolor{DS2f8}{ 5.0} &  \cellcolor{DS2b9} \textcolor{DS2f9}{ 14.0} &  \cellcolor{DS2b10} \textcolor{DS2f10}{ 32.0} &  \cellcolor{DS2b11} \textcolor{DS2f11}{ 18.0}\\ 
YouCook II \cite{ZhXuCoCVPR18}  &  \cellcolor{DS3b0} \textcolor{DS3f0}{ 0.0} &  \cellcolor{DS3b1} \textcolor{DS3f1}{ 1.0} &  \cellcolor{DS3b2} \textcolor{DS3f2}{ 30.0} &  \cellcolor{DS3b3} \textcolor{DS3f3}{ 71.0} &  \cellcolor{DS3b4} \textcolor{DS3f4}{ 45.5} &  \cellcolor{DS3b5} \textcolor{DS3f5}{ 53.7} &  \cellcolor{DS3b6} \textcolor{DS3f6}{ 52.7} &  \cellcolor{DS3b7} \textcolor{DS3f7}{ ~~ } &  \cellcolor{DS3b8} \textcolor{DS3f8}{ 0.0} &  \cellcolor{DS3b9} \textcolor{DS3f9}{ 28.0} &  \cellcolor{DS3b10} \textcolor{DS3f10}{ 39.0} &  \cellcolor{DS3b11} \textcolor{DS3f11}{ 24.0}\\ 
Cross-Task \cite{Zhukov19}  &  \cellcolor{DS4b0} \textcolor{DS4f0}{ 3.5} &  \cellcolor{DS4b1} \textcolor{DS4f1}{ 6.0} &  \cellcolor{DS4b2} \textcolor{DS4f2}{ 31.0} &  \cellcolor{DS4b3} \textcolor{DS4f3}{ 71.5} &  \cellcolor{DS4b4} \textcolor{DS4f4}{ 51.0} &  \cellcolor{DS4b5} \textcolor{DS4f5}{ 56.3} &  \cellcolor{DS4b6} \textcolor{DS4f6}{ 55.0} &  \cellcolor{DS4b7} \textcolor{DS4f7}{ ~~ } &  \cellcolor{DS4b8} \textcolor{DS4f8}{ 2.0} &  \cellcolor{DS4b9} \textcolor{DS4f9}{ 31.0} &  \cellcolor{DS4b10} \textcolor{DS4f10}{ 32.0} &  \cellcolor{DS4b11} \textcolor{DS4f11}{ 19.0}\\ 
\bottomrule \end{tabular}}

==> mlhc-submission-files/extra_tables.tex <==



\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_chf} Summary of Results - Bias AUROC for pna}
\scalebox{0.4}{
\begin{tabular}{c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U}    & -- &  -- \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u   & -- &  -- \\
            \hspace{10mm} b+/b-  & -- &  -- \\
            \hspace{10mm} b+/b+  & -- &  -- \\
\hline 
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & -- &  -- \\
            \hspace{10mm} b+/b-  & -- &  -- \\
            \hspace{10mm} b+/b+   & -- &  -- \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{Age AUROC (95\% CI)} \\
 \midrule
   & -- &  -- \\
 \hline
  \\ 
    & -- &   0.74 (0.62-0.84) \\
     & -- &  -- \\
    & -- &  -- \\
\hline
  \\ 
    & -- &   0.68 (0.56-0.79) \\
     & -- &  -- \\
     & -- &  -- \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Sex}} \\ & \textbf{N train} & \textbf{BIas AUROC (95\% CI)} \\
 \midrule
   & -- &  0.84(0.75 - 0.91) \\
 \hline
  \\ 
    & -- & 0.76 (0.66-0.85) \\
    & -- & -- \\
    & -- & --
 \\
\hline
  \\ 
    & -- & 0.72 (0.62-0.83)\\
    & -- & -- \\
    & -- & -- \\
 \bottomrule
\end{tabular}

}
\end{table*}




\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_chf} Summary of Results - TPR Disparity of CHF}
\scalebox{0.4}{
\begin{tabular}{c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U}   & -- & 0.55 \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u  & -- & 0.35 \\
            \hspace{10mm} b+/b- & -- & -- \\
            \hspace{10mm} b+/b+ & -- & -- \\
\hline
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & -- & 0.47 \\
            \hspace{10mm} b+/b- & -- & -- \\
            \hspace{10mm} b+/b+  & -- & -- \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{CHF TPR Disparity} \\
 \midrule
   & -- & 0.27 \\
 \hline
  \\ 
    & -- & -0.065 \\
    & -- & -- \\
    & -- & -- \\
\hline
  \\ 
    & -- & 0.38 \\
    & -- & -- \\
    & -- & -- \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Sex}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   & -- & 0.52 \\
 \hline
  \\ 
    & -- & 0.40 \\
    & -- & -- \\
    & -- & -- \\
\hline
  \\ 
    & -- & -0.05 \\
    & -- & -- \\
    & -- & -- \\
 \bottomrule
\end{tabular}



\begin{tabular}{c c c}
\toprule
& & \multicolumn{1}{c}{\textbf{Bias type: Race}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   & -- & -- \\
\hline
  \\ 
    & -- & -- \\
    & -- & -- \\
    & -- & -- \\
\hline
  \\ 
    & -- & -- \\
    & -- & -- \\
    & -- & -- \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Pacemaker}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   & -- & -- \\
 \hline
  \\ 
    & -- & -- \\
    & -- & -- \\
    & -- & -- \\
\hline
  \\ 
    & -- & -- \\
    & -- & -- \\
    & -- & -- \\
 \bottomrule
\end{tabular}

}
\end{table*}





==> mlhc-submission-files/tables.tex <==
% CHF Biased/Pna Unbiased results - all 



\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_chf} Summary of Results - CHF}
\scalebox{0.4}{
\begin{tabular}{c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U}   & 508 (0.12) & 0.75 (0.65-0.84) \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u  & 508 (0.12) &  \textbf{0.81 (0.72-0.88)}   \\
            \hspace{10mm} b+/b- & 448 (0.27) &  $0.79$ $(0.70-0.87)$ \\
            \hspace{10mm} b+/b+  & 408 (0.11) & \textbf{0.81 (0.72-0.88)} \\
\hline
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & 508 (0.12) &  \textbf{0.81 (0.73-0.89)}  \\
            \hspace{10mm} b+/b- & 448 (0.27) & $0.72$ $(0.62-0.82)$ \\
            \hspace{10mm} b+/b+  & 408 (0.11) & $0.79$ $(0.69-0.88)$ \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   &553 (0.25) & 0.75 (0.65-0.85)\\
 \hline
  \\ 
    & 553 (0.25) & $0.75$ $(0.64-0.85)$ \\
    & 425 (0.39) & $ 0.75$ $(0.65-0.85)$ \\
    & 465 (0.27) & $0.78$ $(0.68-0.87)$  \\
\hline
    \\ 
    & 553 (0.25) & \textbf{0.79 (0.68-0.88)} \\
    & 425 (0.39) & $0.76$ $(0.66-0.85)$ \\
    & 465 (0.27) & $0.83$ $(0.73-0.90)$ \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Sex}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   &  504 (0.13 & 0.66 (0.53-0.78)\\
 \hline
  \\ 
    & 504 (0.13) &\textbf{0.80 (0.71-0.88)} \\
    & 424 (0.24) & $0.73$ $(0.62-0.83)$ \\
    & 400 (0.13) & $0.57$ $(0.46-0.69)$ \\
    
\hline
    \\ 
    & 504 (0.13) & $0.69$ $(0.58-0.80)$ \\
    & 424 (0.24) & $0.62$ $(0.50-0.74)$ \\
    & 400 (0.13) & $0.69$ $(0.58-0.80)$ \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
& & \multicolumn{1}{c}{\textbf{Bias type: Race}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   & 706 (0.012) & 0.44 (0.31-0.56)\\
 \hline
  \\ 
    & 706 (0.012) & \textbf{0.83 (0.75-0.90)} \\
    & 526 (0.05) & \textbf{0.83 (0.73-0.90)} \\
    &   & -- \\
\hline
    \\ 
    & 706 (0.012)  & $0.65$ $(0.53-0.76)$  \\
    & 526 (0.05) & $0.80$ $(0.70-0.88)$ \\
    & -- & -- \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Pacemaker}} \\ & \textbf{N train} & \textbf{CHF AUROC (95\% CI)} \\
 \midrule
   & 780 (0.06) & 0.76 (0.64-0.86)\\
 \hline
  \\ 
    & 780 (0.06) & $0.82$ $(0.73-0.90)$ \\
    & 504 (0.10) & $0.83$ $(0.75-0.91)$ \\
    & $604$ $(0.08)$ & $0.82$ $(0.74-0.89)$ \\
\hline
    \\ 
    & 780 (0.06) & $0.80$ $(0.71-0.88)$ \\
    & 504 (0.10) & $0.83$ $(0.75-0.90)$ \\
    & $604$ $(0.08)$ & \textbf{0.84 (0.76-0.91)}\\
 \bottomrule
\end{tabular}

}
\end{table*}



\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_chf} Summary of Results - CHF Bias AUROC}
\scalebox{0.4}{
\begin{tabular}{c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U}   & -- & 0.78 (0.68-0.86) \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u  & -- & 0.70 (0.60-0.80) \\
            \hspace{10mm} b+/b- & -- & 0.74 (0.65-0.83) \\
            \hspace{10mm} b+/b+ & -- & 0.71 (0.61-0.80) \\
\hline 
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & -- & 0.71 (0.61-0.80) \\
            \hspace{10mm} b+/b- & -- & 0.77 (0.68-0.86) \\
            \hspace{10mm} b+/b+  & -- & 0.70 (0.61-0.79) \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
   & -- & 0.77 (0.68-0.86) \\
 \hline
  \\ 
    & -- & 0.70 (0.58-0.81) \\
    & -- & 0.67 (0.49-0.82) \\
    & -- &  0.74 (0.64-0.84) \\
\hline
  \\ 
    & -- &  0.70 (0.59-0.81)  \\
    & -- & 0.80 (0.72-0.88) \\
    & -- &  0.70 (0.59-0.80) \\
 \bottomrule
\end{tabular}


\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Sex}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
   & -- &  0.88 (0.80-0.94) \\
 \hline
  \\ 
    & -- & 0.67 (0.56-0.78) \\
    & -- & 0.82 (0.73-0.89) \\
    & -- & 0.61 (0.44-0.76)
 \\
\hline
  \\ 
    &0.77 (0.67-0.87) \\
    & -- & 0.73 (0.63 - 0.82) \\
    & -- & 0.70 (0.59-0.81) \\
 \bottomrule
\end{tabular}

}
\end{table*}









\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_pna} Summary of Results - Pneumonia}
\scalebox{0.4}{
\begin{tabular}{c c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{Pneumonia AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U} & $476$ $(0.20)$   & 0.60 (0.45-0.73) \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u & $476$ $(0.20)$  & 0.57 (0.42-0.72) \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ & $0.59$ $(0.44-0.74)$ \\
            \hspace{10mm} b+/b+ & $404$ $(0.17)$ & 0.56 (0.42-0.70)  \\
\hline
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & $476$ $(0.20)$  & $0.56$ $(0.41-0.69)$ \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ & $0.57$ $(0.43-0.71)$\\
            \hspace{10mm} b+/b+  & $404$ $(0.17)$ & \textbf{0.62 (0.48-0.75)} \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{Pneumoonia AUROC (95\% CI)} \\
 \midrule
  & $447$ $(0.32)$ & 0.58 (0.43-0.72) \\
 \hline
  \\ 
    & $447$ $(0.32)$ & 0.59 (0.46-0.72) \\
    & $411$ $(0.28)$  & $0.63$ $(0.48-0.77)$ \\
    & $463$ $(0.27)$ & $0.59 (0.45 - 0.71)$ \\
\hline
    \\ 
    & $447$ $(0.32)$ & $0.59$ $(0.46-0.72)$ \\
    & $411$ $(0.28)$  & $0.63$ $(0.49-0.77)$ \\
    & $463$ $(0.27)$ & $0.60$ $(0.47-0.72)$ \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Gender}} \\ & \textbf{N train} & \textbf{Pneumonia AUROC (95\% CI)} \\
 \midrule
       & $480$ $(0.15)$ & 0.61 (0.42-0.75) \\

 \hline
  \\ 
     & $480$ $(0.15)$ & $0.73$ $(0.62-0.83)$ \\
    & $464$ $(0.20)$ & $0.68$ $(0.52-0.81)$ \\
    & $400$ $(0.17)$ & $0.57$ $(0.38-0.75)$ \\
    
\hline
    \\ 
    & $480$ $(0.15)$ & $0.73$ $(0.59-0.83)$ \\
    & $464$ $(0.20)$ & $0.68$ $(0.51-0.82)$ \\
    & $400$ $(0.17)$ & \textbf{0.74 (0.61-0.85)} \\
 \bottomrule
\end{tabular}
}
\end{table*}




\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_pna_bias} Summary of Results - Pneumonia Bias AUROC}
\scalebox{0.4}{
\begin{tabular}{c c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U} & $476$ $(0.20)$   &  0.77 (0.67-0.86) \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u & $476$ $(0.20)$  & $0.74 (0.65-0.83)$ \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ & $0.75 (0.65-0.84)$\\
            \hspace{10mm} b+/b+ & $404$ $(0.17)$ &  $0.75 (0.66-0.84)$ \\
\hline
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & $476$ $(0.20)$  & $0.78$ $(0.69-0.86)$ \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ &  $0.72 (0.64-0.80)$ \\
            \hspace{10mm} b+/b+  & $404$ $(0.17)$ &  $0.71 (0.62-0.80)$\\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
  & $447$ $(0.32)$ & 0.74 (0.63-0.84) \\
 \hline
  \\ 
    & $447$ $(0.32)$ & 0.72 (0.61-0.83) \\
    & $411$ $(0.28)$  & 0.72 (0.61-0.82) \\
    & $463$ $(0.27)$ & 0.71 (0.60-0.82)\\
\hline
    \\ 
    & $447$ $(0.32)$ & 0.68 (0.57-0.79) \\
    & $411$ $(0.28)$  & 0.70 (0.60-0.80) \\
    & $463$ $(0.27)$ & 0.71 (0.59-0.82) \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Gender}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
       & $480$ $(0.15)$ & $0.81 (0.72-0.89)$ \\

 \hline
  \\ 
     & $480$ $(0.15)$ & $0.70 (0.60-0.81)$ \\
    & $464$ $(0.20)$ & $0.79 (0.69-0.88)$ \\
    & $400$ $(0.17)$ & $0.85 (0.77-0.92)$\\
    
\hline
    \\ 
    & $480$ $(0.15)$ & $0.73 (0.63-0.83)$ \\
    & $464$ $(0.20)$ & $0.69 (0.57-0.80)$ \\
    & $400$ $(0.17)$ & $0.76 (0.66-0.86)$ \\
 \bottomrule
\end{tabular}
}
\end{table*}



\begin{table*}[ht]
    \centering
    \caption{\label{tab:all_results_pna_bias} Summary of Results - Pneumonia Bias AUROC}
\scalebox{0.4}{
\begin{tabular}{c c c c}
\toprule
\textbf{Approach} &  & \multicolumn{1}{c}{\textbf{Bias type: BMI}} \\ & \textbf{N Train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
\textbf{Single Task B/U} & $476$ $(0.20)$   &  0.77 (0.67-0.86) \\
 \hline
\textbf{Multi Task} \\ 
            \hspace{10mm} b/u & $476$ $(0.20)$  & $0.74 (0.65-0.83)$ \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ & $0.75 (0.65-0.84)$\\
            \hspace{10mm} b+/b+ & $404$ $(0.17)$ &  $0.75 (0.66-0.84)$ \\
\hline
\textbf{2-Stage} \\ 
            \hspace{10mm} b/u  & $476$ $(0.20)$  & $0.78$ $(0.69-0.86)$ \\
            \hspace{10mm} b+/b- & $455$ $(0.17)$ &  $0.72 (0.64-0.80)$ \\
            \hspace{10mm} b+/b+  & $404$ $(0.17)$ &  $0.71 (0.62-0.80)$\\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Age}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
  & $447$ $(0.32)$ & 0.74 (0.63-0.84) \\
 \hline
  \\ 
    & $447$ $(0.32)$ & 0.72 (0.61-0.83) \\
    & $411$ $(0.28)$  & 0.72 (0.61-0.82) \\
    & $463$ $(0.27)$ & 0.71 (0.60-0.82)\\
\hline
    \\ 
    & $447$ $(0.32)$ & 0.68 (0.57-0.79) \\
    & $411$ $(0.28)$  & 0.70 (0.60-0.80) \\
    & $463$ $(0.27)$ & 0.71 (0.59-0.82) \\
 \bottomrule
\end{tabular}

\begin{tabular}{c c c}
\toprule
&  & \multicolumn{1}{c}{\textbf{Bias type: Gender}} \\ & \textbf{N train} & \textbf{Bias AUROC (95\% CI)} \\
 \midrule
       & $480$ $(0.15)$ & $0.81 (0.72-0.89)$ \\

 \hline
  \\ 
     & $480$ $(0.15)$ & $0.70 (0.60-0.81)$ \\
    & $464$ $(0.20)$ & $0.79 (0.69-0.88)$ \\
    & $400$ $(0.17)$ & $0.85 (0.77-0.92)$\\
    
\hline
    \\ 
    & $480$ $(0.15)$ & $0.73 (0.63-0.83)$ \\
    & $464$ $(0.20)$ & $0.69 (0.57-0.80)$ \\
    & $400$ $(0.17)$ & $0.76 (0.66-0.86)$ \\
 \bottomrule
\end{tabular}
}
\end{table*}



\begin{table}[htbp]
    \centering
    \caption{Correlations and splits - CHF \dfnote{This is too small; few will read it although it's nice to have. This might fit in supplemental, an appendix, or something else. You should think about showing this as a heatmap or showing only the most important subset of information (e.g., only train/val). Essentially, I should be able to glance at the table and get this very quickly; it's quite hard here. - Working on this on 3/27} }
    \label{tab:chf_correlations_splits_chf}
    \scalebox{0.5}{
    \begin{tabular}{c c c c c }
        \toprule
\multirow{\textbf{Task}} & \multicolumn{2}{c}{\textbf{B/U Correlation}} & \multicolumn{2}{c}{\textbf{B/U  Split}}\\
    & \textbf{CHF} & \textbf{Pneumonia} &  \textbf{CHF} & \textbf{Pneumonia} \\
         \midrule
         \textbf{BMI} \\ 
            \hspace{10mm} Train  & 0.99 & -0.003 & $508$ $(0.12)$ & $508$ $(0.35)$ \\
            \hspace{10mm} Validation & 1.0 & -0.007 & $127$ $(0.13)$ & $127$ $(0.36)$\\
            \hspace{10mm} Test & -0.01 & 0.004 & $111$ $(0.23)$ & $111$ $(0.14)$\\
        \hline
        \textbf{Age} \\ 
            \hspace{10mm} Train  & 1.0 & 0.003 & $553$ $(0.25)$ & $553$ $(0.29)$\\
            \hspace{10mm} Validation & 0.99 & -0.02 & $139$ $(0.19)$ & $139$ $(0.32)$\\
            \hspace{10mm} Test & -0.02& 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$\\
         \hline
         \textbf{Sex} \\ 
            \hspace{10mm} Train  & 1.0 & -0.02 & $504$ $(0.13)$ & $504$ $(0.32)$\\
            \hspace{10mm} Validation & 1.0 & 0.02 & $127$ $(0.10)$ & $127$ $(0.35)$\\
            \hspace{10mm} Test & -0.02 & 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$\\
         \hline
        \textbf{Race} \\
        \hspace{10mm} Train  & 1.0 & 0.004 & $706$ $(0.012)$ & $706$ $(0.32)$\\
            \hspace{10mm} Validation & 1.0 & -0.01 & $177$ $(0.02)$ & $177$ $(0.27)$\\
            \hspace{10mm} Test & -- & -- & $111$ $(0.23)$ & $111$ $(0.14)$\\
            
         \hline
         \textbf{Pacemaker} \\ 
            \hspace{10mm} Train  & 0.99 & -0.02 & $780$ $(0.06)$ & $780$ $(0.31)$\\
            \hspace{10mm} Validation & 0.99 & -0.02 & $195$ $(0.06)$ & $195$ $(0.33)$\\
            \hspace{10mm} Test & -- & -- & $111$ $(0.23)$ & $111$ $(0.14)$\\
         \bottomrule
        \end{tabular}
        
        \begin{tabular}{c c c c }
        \toprule
        \multicolumn{2}{c}{\textbf{B+/B- Correlation}} & \multicolumn{2}{c}{\textbf{B+/B- Split}}\\
        \textbf{CHF} & \textbf{Pneumonia} &  \textbf{CHF} & \textbf{Pneumonia} \\
         \midrule 
         \\
            1.00 & -0.27 & $448$ $(0.27)$ & $448$ $(0.40)$ \\
            1.00 & -0.31 & $112$ $(0.29)$ & $112$ $(0.39)$ \\
            -0.01 & 0.00 & $111$ $(0.23)$ & $111$ $(0.14)$\\
        \hline
        \\
            1.00 & -0.25 & $425$ $(0.39)$ & $425$ $(0.40)$ \\
            1.00 & -0.25 & $107$ $(0.38)$ & $107$ $(0.37)$ \\
            -0.02 & 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$\\
         \hline
         \\
            1.00 & -0.23 & $424$ $(0.24)$ & $424$ $(0.38)$ \\
            1.00 & -0.21 & $107$ $(0.24)$ & $107$ $(0.41)$ \\
            -0.02 & 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$ \\
         \hline
         \\
            1.00 & -0.15 & $526$ $(0.05)$ & $526$ $(0.43)$ \\
            1.00 & -0.15 & $132$ $(0.08)$ & $132$ $(0.36)$ \\
            -- & -- & $111$ $(0.23)$ & $111$ $(0.14)$ \\
            
         \hline
         \\
            0.99 & -0.16 & $504$ $(0.10)$ & $504$ $(0.49)$ \\
            1.00 & -0.14 & $126$ $(0.06)$ & $126$ $(0.43)$ \\
            -- & -- & $111$ $(0.23)$ & $111$ $(0.14)$ \\
         \bottomrule
        \end{tabular}
        
        \begin{tabular}{c c c c }
        \toprule
        \multicolumn{2}{c}{\textbf{B+/B+ Correlation}} & \multicolumn{2}{c}{\textbf{B+/B+ Split}}\\
        \textbf{CHF} & \textbf{Pneumonia} &  \textbf{CHF} & \textbf{Pneumonia} \\
         \midrule 
         \\
            1.00 & 0.21 & $408$ $(0.11)$ & $408$ $(0.25)$ \\
            1.00 & 0.22 & $102$ $(0.08)$ & $102$ $(0.20)$ \\
            -0.01 & 0.00 & $111$ $(0.23)$ & $111$ $(0.14)$ \\
        \hline
        \\
            1.00 & 0.22 & $465$ $(0.27)$ & $465$ $(0.20)$ \\
            1.00 & 0.16 & $117$ $(0.26)$ & $117$ $(0.14)$ \\
            -0.02 & 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$ \\
         \hline
         \\
            1.00 & 0.20 & $400$ $(0.13)$ & $400$ $(0.19)$ \\
            1.00 & 0.21 & $101$ $(0.14)$ & $101$ $(0.12)$ \\
            -0.02 & 0.02 & $111$ $(0.23)$ & $111$ $(0.14)$ \\
         \hline
         \\
            -- & -- & -- & -- \\
            -- & -- & -- & -- \\
            -- & -- & -- & -- \\
            
         \hline
         \\
            0.99 & 0.13 & $604$ $(0.08)$ & $604$ $(0.10)$ \\
            1.00 & 0.13 & $151$ $(0.05)$ & $151$ $(0.09)$ \\
            -- & -- & $111$ $(0.23)$ & $111$ $(0.14)$ \\
         \bottomrule
        \end{tabular}}
    \label{tab:shortcut_tasks}
\end{table}
